PP-SAM: Perturbed Prompts for Robust Adaptation of Segment Anything Model for Polyp Segmentation

The Segment Anything Model (SAM), originally designed for general-purpose segmentation tasks, has been used recently for polyp segmentation. Nonetheless, fine-tuning SAM with data from new imaging centers or clinics poses significant challenges. This is because this necessitates the creation of an expensive and time-intensive annotated dataset, along with the potential for variability in user prompts during inference. To address these issues, we propose a robust fine-tuning technique, PP-SAM, that allows SAM to adapt to the polyp segmentation task with limited images. To this end, we utilize variable perturbed bounding box prompts (BBP) to enrich the learning context and enhance the model's robustness to BBP perturbations during inference. Rigorous experiments on polyp segmentation benchmarks reveal that our variable BBP perturbation significantly improves model resilience. Notably, on Kvasir, 1-shot fine-tuning boosts the DICE score by 20% and 37% with 50 and 100-pixel BBP perturbations during inference, respectively. Moreover, our experiments show that 1-shot, 5-shot, and 10-shot PP-SAM with 50-pixel perturbations during inference outperform a recent state-of-the-art (SOTA) polyp segmentation method by 26%, 7%, and 5% DICE scores, respectively. Our results motivate the broader applicability of our PP-SAM for other medical imaging tasks with limited samples. Our implementation is available at https://github.com/SLDGroup/PP-SAM.

==> sec/5_ablation_study.tex <==
\section{Ablation Studies}
\label{sec:ablation_study}

\begin{table}[t]
\centering 
    {%\small{
\begin{adjustbox}{width=0.48\textwidth}
{\begin{tabular}{lcrrr}
\toprule
Encoders & Decoders    &\multicolumn{1}{c}{\#FLOPs(G)} & \multicolumn{1}{c}{\#Params(M)} & \multicolumn{1}{l}{DICE (\%)} \\
\midrule
   PVTv2-B0      & CASCADE &  0.439 &  2.32 &  80.54 \\
   PVTv2-B0    & EMCAD (\textbf{Ours})    & \textbf{0.110} &  \textbf{0.507} & \textbf{81.05}   \\
\midrule 
  PVTv2-B2     & CASCADE &  1.93 & 9.27 & 82.78     \\
  PVTv2-B2   & EMCAD (\textbf{Ours}) & \textbf{0.381} & \textbf{1.91}     & \textbf{83.16}   \\
\bottomrule %\\
\end{tabular}}
\end{adjustbox}

}%}
\vspace{-0.1cm}
\caption{Comparison with the baseline decoder on Synapse Multi-organ dataset. We only report the \#FLOPs (with input resolution of $224\times224$) and the \#parameters of the decoders. All the results are averaged over five runs. Best results are shown in bold.}
\vspace{-0.3cm}
\label{tab:compare_baseline_decoder}
\end{table}
%------------------------------------------------------------------------- 

%\subsection{Transfer learning experiments}
%\subsection{Different encoders}
%\subsection{Small model and decoder}
%\subsection{Compare with other decoders}


In this section, we conduct ablation studies to explore different aspects of our architectures and the experimental framework. More ablations are in supplementary \cref{asec:ablation}.

% from other paper
%In Table 4, the CASCADE performs the best with the MiT. We believe that this is because the convolution operation inside MiT can maintain the consistency of the spatial information of the model. Furthermore, the experiments in Table 5 demonstrate the effectiveness of the CASCADE and its components.

%\textbf{Effective enhancement/refinement of features.}
%We visualize the features of our CASCADE, as well as Cascaded Upsampler (CUP) \cite{chen2021transunet} in Figure \ref{fig:middle_features}. We compute the average of all channels in the feature map and then produce the heatmap using OpenCV-Python. It is evident from Figure \ref{fig:middle_features} that the attention mechanism used in our CASCADE helps identify, enhance, and group the pixels better than CUP.  

\subsection{Effect of different components of EMCAD}
We conduct a set of experiments on the Synapse multi-organ dataset to understand the effect of different components of our EMCAD decoder. We start with only the encoder and add different modules such as Cascaded structure, LGAG, and MSCAM to understand their effect. Table \ref{tab:ablation_components} exhibits that the cascaded structure of the decoder helps to improve performance over the non-cascaded one. The incorporation of LGAG and MSCAM improves performance, however, MSCAM proves to be more effective. When both the LGAG and MSCAM modules are used together, it produces the best DICE score of 83.16\%. It is also evident that there is about 3.06\% improvement in the DICE score with an additional 0.381G FLOPs and 1.91M parameters.   

\subsection{Effect of multi-scale kernels in MSCAM}
We have conducted another set of experiments on Synapse multi-organ and ClinicDB datasets to understand the effect of different multi-scale kernels used for depth-wise convolutions in MSDC. Table \ref{tab:multi_kernels} reports these results which show that performance improves from $1\times1$ to $3\times3$ kernel. When $1\times1$ kernel is used together with $3\times3$ it improves more than when using them alone. However, when two $3\times3$ kernels are used together, performance drops. The incorporation of a $5\times5$ kernel with $1\times1$ and $3\times3$ kernels further improves the performance and it achieves the best results in both Synapse multi-organ and ClinicDB datasets. If we add additional larger kernels (e.g., $7\times7$, $9\times9$), the performance of both datasets drops. Based on these empirical observations, we choose $[1,3,5]$ kernels in all our experiments. %Based on these empirical observations, we choose $[1,3,5]$ kernels for all the binary segmentation tasks and $[1,3,5,7]$ kernels for multi-class segmentation tasks. %Nonetheless, it improves the performance of the Synapse multi-organ dataset. If we have another large kernel, it reduces the performances of both datasets.   
 

\subsection{Comparison with the baseline decoder}

In Table \ref{tab:compare_baseline_decoder}, we report the experimental results with the computational complexity of our EMCAD decoder and a baseline decoder, namely CASCADE. From Table \ref{tab:compare_baseline_decoder}, we can see that our EMCAD decoder with PVTv2-B2 requires 80.3\% fewer FLOPs and 79.4\% fewer parameters to outperform (by 0.38\%) the respective CASCADE decoder. Similarly, our EMCAD decoder with PVTv2-B0 achieves 0.5\% better DICE score than the CASCADE decoder with 78.1\% fewer parameters and 74.9\% fewer FLOPs.        

%\subsection{Qualitative results}


